PolyFootNet: Extracting Polygonal Building Footprints in Off-Nadir Remote Sensing Images

Extracting polygonal building footprints from off-nadir imagery is crucial for diverse applications. Current deep-learning-based extraction approaches predominantly rely on semantic segmentation paradigms and post-processing algorithms, limiting their boundary precision and applicability. However, existing polygonal extraction methodologies are inherently designed for near-nadir imagery and fail under the geometric complexities introduced by off-nadir viewing angles. To address these challenges, this paper introduces Polygonal Footprint Network (PolyFootNet), a novel deep-learning framework that directly outputs polygonal building footprints without requiring external post-processing steps. PolyFootNet employs a High-Quality Mask Prompter to generate precise roof masks, which guide polygonal vertex extraction in a unified model pipeline. A key contribution of PolyFootNet is introducing the Self Offset Attention mechanism, grounded in Nadaraya-Watson regression, to effectively mitigate the accuracy discrepancy observed between low-rise and high-rise buildings. This approach allows low-rise building predictions to leverage angular corrections learned from high-rise building offsets, significantly enhancing overall extraction accuracy. Additionally, motivated by the inherent ambiguity of building footprint extraction tasks, we systematically investigate alternative extraction paradigms and demonstrate that a combined approach of building masks and offsets achieves superior polygonal footprint results. Extensive experiments validate PolyFootNet's effectiveness, illustrating its promising potential as a robust, generalizable, and precise polygonal building footprint extraction method from challenging off-nadir imagery. To facilitate further research, we will release pre-trained weights of our offset prediction module at https://github.com/likaiucas/PolyFootNet.

==> chapters/Acknowledgement.tex <==
\section{Acknowledgements}
\label{sec:Acknowledgement}
This research was funded by the National Key R\&D Program of China under Grant number 2021YFB3900504.

==> chapters/Results.tex <==
\section{Results}
\label{sec:Results}

This section presents the main results obtained in this research, as well as their detailed analysis is performed.

\subsection{Subsection name}
\label{sec:}

\begin{table*}[!h]
\caption{An example of a simple table containing descriptive statistics.}
\label{tab:tab_descr_1}
\setlength{\arrayrulewidth}{1.05 pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular*}{1.0\textwidth}{@{\extracolsep{\fill}}lrr}
\hline
Parameter & Column Name & Column Name \\
\hline
Mean, $\mu$ & 0.79 & 0.98 \\
\hline
\end{tabular*}
\begin{spacing}{0.5}
{\scriptsize Note: There are explanations to the table.}
\end{spacing}
\end{table*}

\subsection{Subsection name}
\label{sec:}

\begin{table*}[!h]
\caption{An example of more complicated table containing estimates of the model parameters.}
\label{tab:}
\setlength{\arrayrulewidth}{1.05 pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular*}{1.0\textwidth}{@{\extracolsep{\fill}}lrrr}
\hline
Parameter & \textit{Column Name} & \textit{Column Name} & \textit{Column Name} \\
\hline

\multicolumn{4}{l}{\textit{Group Name}} \\
$\mu$ & 0.30\textsuperscript{***} {\footnotesize (0.01)} & 0.30\textsuperscript{***} {\footnotesize (0.01)} & 0.30\textsuperscript{***} {\footnotesize (0.01)} \\
$\phi$ & 0.30\textsuperscript{***} {\footnotesize (0.01)} & 0.30\textsuperscript{***} {\footnotesize (0.01)} & 0.30\textsuperscript{***} {\footnotesize (0.01)} \\

\multicolumn{4}{l}{\textit{Group Name}} \\
$\mu$ & 0.40\textsuperscript{*} {\footnotesize (0.17)} & 0.40\textsuperscript{*} {\footnotesize (0.17)} & 0.40\textsuperscript{*} {\footnotesize (0.17)} \\
$\phi$ & 0.40\textsuperscript{*} {\footnotesize (0.17)} & 0.40\textsuperscript{*} {\footnotesize (0.17)} & 0.40\textsuperscript{*} {\footnotesize (0.17)} \\

\hline
\end{tabular*}
\begin{spacing}{0.5}
{\scriptsize Note: Standard errors of coefficients are given in parentheses. The levels of significance notation: *** -- 1\%, ** -- 5\%, * -- 10\%.}
\end{spacing}
\end{table*}

% \subsection{Subsection name}
% \label{sec:}

% \begin{figure*}[!h]
% \centering
% \includegraphics[width=1.0\textwidth,keepaspectratio]{Figure}
% \caption{Figure Title.}
% \label{fig:}
% \end{figure*}

==> chapters/Title.tex <==
%% title
\title{OBMv2: Extracting polygonal footprints in off-nadir images with multi-level information system}%\tnoteref{titlenote}
% \tnotetext[titlenote]{Comment to the article. Such comments may be several.}

%% authors & affiliations
\author[1,2,3]{Kai Li}
\author[1]{Yupeng Deng}
\author[1]{Jingbo Chen}
\author[1]{Yu Meng\corref{corrauthor}}
\author[1]{Zhihao Xi}
\author[1,3]{Junxian Ma}
\author[1,3]{Chenhao Wang}
\author[2]{Xiangyu Zhao}
% \author{Kai Li}




\cortext[corrauthor]{Yu Meng is the corresponding author. 
\\This research was funded by the National Key R\&D Program of China under Grant number 2021YFB3900504. 
\\Here is information on the communication with Kai Li, which will be interact with the journal editors. \url{likai211@mails.ucas.ac.cn}}
% \ead{email\_author2@domen.ru}
\address[1]{Aerospace Information Research Institute, Chinese Academy of Sciences, Beijing 100101, China}
\address[2]{School of Data Science, City University of Hong Kong, Hong Kong 999077, China}
\address[3]{School of Electronic Electrical and Communication Engineering, University of Chinese Academy of Sciences, Beijing 100049, China}


% \affiliation[1]{organization={Aerospace Information Research Institute, Chinese Academy of Sciences},
%             addressline={9 Dengzhuang South Road},%, Haidian District
%             city={Beijing},
%             postcode={100094}, 
%             % state={},
%             country={China}}
% \affiliation[2]{organization={School of Electronic, Electrical and Communication Engineering, University of Chinese Academy of Sciences},
%             addressline={19 Yuquan Road},%, Shijingshan District
%             city={Beijing},
%             postcode={100049}, 
%             % state={},
%             country={China}}
% \affiliation[3]{organization={School of Data Science,City University of Hong Kong},
%             addressline={Kowloon Tong},
%             city={Hong Kong},
%             postcode={999077}, 
%             % state={},
%             country={China}}
